Decision Making of Maximizers and Satisficers Based on Collaborative Explanations

Rating-based summary statistics are ubiquitous in e-commerce, and often are crucial components in personalized recommendation mechanisms. Largely left unexplored, however, is the issue to what extent the descriptives of rating distributions influence the decision making of online consumers. We conducted a conjoint experiment to explore how different summarizations of rating distributions (i.e., in the form of the number of ratings, mean, variance, skewness or the origin of the ratings) impact users' decision making. Results from over 200 participants indicate that users are primarily guided by the mean and the number of ratings and to a lesser degree by the variance, and the origin of a rating. We also looked into the maximizing behavioral tendencies of our participants, and found that in particular participants scoring high on the Decision Difficulty subscale displayed other sensitivities regarding the way in which rating distributions were summarized than others.

==> plot/mch1.tex <==
% Created by tikzDevice version 0.11 on 2018-05-07 22:45:06
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (216.81,216.81);
\end{scope}
\begin{scope}
\path[clip] ( 34.77, 70.56) rectangle (211.31,174.09);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 34.77, 70.56) rectangle (211.31,174.09);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.77, 89.25) --
	(211.31, 89.25);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.77,117.22) --
	(211.31,117.22);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.77,145.19) --
	(211.31,145.19);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.77,173.15) --
	(211.31,173.15);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.77, 75.27) --
	(211.31, 75.27);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.77,103.24) --
	(211.31,103.24);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.77,131.20) --
	(211.31,131.20);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.77,159.17) --
	(211.31,159.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 51.85, 70.56) --
	( 51.85,174.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 80.33, 70.56) --
	( 80.33,174.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (108.80, 70.56) --
	(108.80,174.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (137.28, 70.56) --
	(137.28,174.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (165.75, 70.56) --
	(165.75,174.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (194.23, 70.56) --
	(194.23,174.09);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] ( 51.85, 75.27) rectangle ( 58.97,131.74);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] ( 44.73, 75.27) rectangle ( 51.85,148.77);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] ( 80.33, 75.27) rectangle ( 87.45,169.39);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] ( 73.21, 75.27) rectangle ( 80.33,148.77);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] (108.80, 75.27) rectangle (115.92,123.67);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] (101.68, 75.27) rectangle (108.80,134.43);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] (137.28, 75.27) rectangle (144.39,127.71);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] (130.16, 75.27) rectangle (137.28,120.09);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] (165.75, 75.27) rectangle (172.87,123.67);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] (158.63, 75.27) rectangle (165.75,123.67);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] (194.23, 75.27) rectangle (201.34, 99.47);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] (187.11, 75.27) rectangle (194.23,102.16);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.82, 72.24) {0.0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.82,100.21) {0.2};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.82,128.17) {0.4};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.82,156.14) {0.6};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.02, 75.27) --
	( 34.77, 75.27);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.02,103.24) --
	( 34.77,103.24);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.02,131.20) --
	( 34.77,131.20);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.02,159.17) --
	( 34.77,159.17);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 51.85, 67.81) --
	( 51.85, 70.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 80.33, 67.81) --
	( 80.33, 70.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] (108.80, 67.81) --
	(108.80, 70.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] (137.28, 67.81) --
	(137.28, 70.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] (165.75, 67.81) --
	(165.75, 70.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] (194.23, 67.81) --
	(194.23, 70.56);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,rotate= 45.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 56.14, 61.33) {Mean*};

\node[text=drawColor,rotate= 45.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 84.61, 61.33) {Number ratings*};

\node[text=drawColor,rotate= 45.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (113.09, 61.33) {High to low};

\node[text=drawColor,rotate= 45.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (141.56, 61.33) {Distribution};

\node[text=drawColor,rotate= 45.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (170.04, 61.33) {Origin};

\node[text=drawColor,rotate= 45.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (198.51, 61.33) {Gut feeling};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 13.08,122.33) {Selected(\%)};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 81.21,185.47) rectangle (164.87,211.31);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{gray}{0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] ( 90.51,191.17) rectangle (104.97,205.62);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{248,118,109}

\path[fill=fillColor] ( 91.22,191.88) rectangle (104.26,204.91);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{gray}{0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (126.91,191.17) rectangle (141.36,205.62);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{RGB}{0,191,196}

\path[fill=fillColor] (127.62,191.88) rectangle (140.65,204.91);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (106.77,195.36) {High};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (143.17,195.36) {Low};
\end{scope}
\end{tikzpicture}


==> plot/mch2.tex <==
% Created by tikzDevice version 0.11 on 2018-05-07 15:03:30
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,180.67);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (216.81,180.67);
\end{scope}
\begin{scope}
\path[clip] ( 34.27, 82.25) rectangle (211.31,175.17);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 34.27, 82.25) rectangle (211.31,175.18);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.27, 99.08) --
	(211.31, 99.08);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.27,124.30) --
	(211.31,124.30);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.27,149.52) --
	(211.31,149.52);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.27,174.73) --
	(211.31,174.73);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.27, 86.48) --
	(211.31, 86.48);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.27,111.69) --
	(211.31,111.69);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.27,136.91) --
	(211.31,136.91);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.27,162.13) --
	(211.31,162.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 49.02, 82.25) --
	( 49.02,175.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 73.61, 82.25) --
	( 73.61,175.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 98.20, 82.25) --
	( 98.20,175.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] (122.79, 82.25) --
	(122.79,175.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] (147.38, 82.25) --
	(147.38,175.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] (171.97, 82.25) --
	(171.97,175.17);

\path[draw=drawColor,line width= 0.6pt,line join=round] (196.56, 82.25) --
	(196.56,175.17);
\definecolor{fillColor}{gray}{0.35}

\path[fill=fillColor] ( 42.87, 86.48) rectangle ( 55.17,170.95);

\path[fill=fillColor] ( 67.46, 86.48) rectangle ( 79.76,110.43);

\path[fill=fillColor] ( 92.05, 86.48) rectangle (104.35, 99.08);

\path[fill=fillColor] (116.64, 86.48) rectangle (128.94,126.82);

\path[fill=fillColor] (141.23, 86.48) rectangle (153.53,128.08);

\path[fill=fillColor] (165.82, 86.48) rectangle (178.11, 94.04);

\path[fill=fillColor] (190.41, 86.48) rectangle (202.70,162.13);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.32, 83.45) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.32,108.66) {20};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.32,133.88) {40};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.32,159.10) {60};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.52, 86.48) --
	( 34.27, 86.48);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.52,111.69) --
	( 34.27,111.69);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.52,136.91) --
	( 34.27,136.91);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.52,162.13) --
	( 34.27,162.13);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 49.02, 79.50) --
	( 49.02, 82.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 73.61, 79.50) --
	( 73.61, 82.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 98.20, 79.50) --
	( 98.20, 82.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] (122.79, 79.50) --
	(122.79, 82.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] (147.38, 79.50) --
	(147.38, 82.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] (171.97, 79.50) --
	(171.97, 82.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] (196.56, 79.50) --
	(196.56, 82.25);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 55.08, 77.30) {all users};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 79.67, 77.30) {did not care};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (104.26, 77.30) {did not unders.};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (128.85, 77.30) {gut feeling};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (153.44, 77.30) {not noticed};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (178.03, 77.30) {other};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (202.62, 77.30) {similar users};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 13.08,128.71) {Frequency};
\end{scope}
\end{tikzpicture}


==> plot/plot_relative_pref.tex <==
% \begin{figure}
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%   width=7cm,
%   height=5cm,
%     ybar,
%     ylabel={Relative preference (\%)},
%     axis y line*=left,    
%     axis x line*=bottom,
%     ymin=0,
%     symbolic x coords={Origin, Rt., Mean, Var., Skew.},
%     xtick=data,
%     nodes near coords,
%     nodes near coords align={vertical},
%     ]
% \addplot[fill=forestgreen, draw=forestgreen] coordinates {(Origin, 14) (Rt., 36) (Mean, 55) (Var., 8)(Skew.,2)};
% \end{axis}
% \end{tikzpicture}
% \caption{Relative preference weight for the attributes of the study.}
% \label{fig:relpref}
% \end{figure}

\begin{figure}
\centering

% Created by tikzDevice version 0.11 on 2018-05-01 18:22:16
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (231.26,144.54);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (231.26,144.54);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] ( -0.00,  0.00) rectangle (231.26,144.54);
\end{scope}
\begin{scope}
\path[clip] ( 60.01, 32.09) rectangle (225.76,139.04);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 60.01, 32.09) rectangle (225.76,139.04);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 93.31, 32.09) --
	( 93.31,139.04);

\path[draw=drawColor,line width= 0.3pt,line join=round] (144.83, 32.09) --
	(144.83,139.04);

\path[draw=drawColor,line width= 0.3pt,line join=round] (196.36, 32.09) --
	(196.36,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 60.01, 44.43) --
	(225.76, 44.43);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 60.01, 65.00) --
	(225.76, 65.00);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 60.01, 85.56) --
	(225.76, 85.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 60.01,106.13) --
	(225.76,106.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 60.01,126.70) --
	(225.76,126.70);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.55, 32.09) --
	( 67.55,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (119.07, 32.09) --
	(119.07,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (170.60, 32.09) --
	(170.60,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (222.12, 32.09) --
	(222.12,139.04);
\definecolor{fillColor}{RGB}{34,139,34}

\path[fill=fillColor] ( 67.55, 38.26) rectangle (103.97, 50.60);

\path[fill=fillColor] ( 67.55, 58.82) rectangle (160.55, 71.17);

\path[fill=fillColor] ( 67.55, 79.39) rectangle (210.50, 91.73);

\path[fill=fillColor] ( 67.55, 99.96) rectangle ( 87.44,112.30);

\path[fill=fillColor] ( 67.55,120.53) rectangle ( 72.70,132.87);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.85] at (111.70, 42.81) {14\%};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.85] at (168.28, 63.38) {36\%};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.85] at (218.23, 83.95) {55\%};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.85] at ( 95.16,104.51) {8\%};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.85] at ( 80.43,125.08) {2\%};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (231.26,144.54);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 55.06, 41.40) {Origin};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 55.06, 61.96) {\# of ratings};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 55.06, 82.53) {Mean};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 55.06,103.10) {Variance};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 55.06,123.67) {Skewness};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (231.26,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 57.26, 44.43) --
	( 60.01, 44.43);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 57.26, 65.00) --
	( 60.01, 65.00);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 57.26, 85.56) --
	( 60.01, 85.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 57.26,106.13) --
	( 60.01,106.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 57.26,126.70) --
	( 60.01,126.70);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (231.26,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.55, 29.34) --
	( 67.55, 32.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (119.07, 29.34) --
	(119.07, 32.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (170.60, 29.34) --
	(170.60, 32.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (222.12, 29.34) --
	(222.12, 32.09);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (231.26,144.54);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 67.55, 21.08) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (119.07, 21.08) {20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (170.60, 21.08) {40};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (222.12, 21.08) {60};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (231.26,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (142.89,  8.00) {Relative preference (\%)};
\end{scope}
\end{tikzpicture}




\caption{Relative preference weight for the attributes of the study.}
\label{fig:relpref}
\end{figure}



==> table/tab_results.tex <==
\begin{table*}[!ht]
\caption{Final results  of the multinomial logit model.}
\begin{tabular}{l ccc ccc ccc}
\toprule
\multirow{2}{*}{Parameter$\beta$	} &	\multicolumn{3}{c}{All Respondents}	&	\multicolumn{3}{c}{Satisficers}	&	\multicolumn{3}{c}{Maximizers}	\\

% \cmidrule(lr){2-4}
% \cmidrule(lr){5-7}
% \cmidrule(lr){8-10}
\cline{2-4}
\cline{5-7}
\cline{8-10}

&	$\beta$	&	Error	&	p-value		&	$\beta$	&	Error	&	p-value	&	$\beta$	&	Error	&	p-value	\\
\midrule
Similar Users	&	0.25	&	0.04	&	<0.05	&	0.27	&	0.06	&	<0.05	&	0.22	&	0.06	&	<0.05	\\
All Users	&	\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}																	\\
70 Ratings	&	0.64	&	0.04	&	<0.05	&	0.73	&	0.06	&	<0.05	&	0.55	&	0.06	&	<0.05	\\
20 Ratings	&	\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}																	\\
Mean 4.3	&	0.98	&	0.05	&	<0.05	&	0.97	&	0.06	&	<0.05	&	0.98	&	0.06	&	<0.05	\\
Mean 3.7	&	\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}																	\\
variance 1.3	&	-0.14	&	0.04	&	<0.05	&	-0.12	&	0.06	&	<0.05	&	-0.15	&	0.06	&	<0.05	\\
variance 0.7	&	\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}																	\\
Skewness -0.5	&	0.04	&	0.04	&	0.40	&	0.06	&	0.06	&	0.29	&	0.01	&	0.06	&	0.89	\\
Skewness -1.2	&	\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}	&\multicolumn{3}{c}{Constrained to 0}							\\										
\bottomrule
\end{tabular}
%\caption{Parameter estimation via the Multinomial logit, on all respondents and on the minimizers and maximizers.}
\label{tab:param_estimate}
\end{table*}

